Skating-Mixer: Long-Term Sport Audio-Visual Modeling with MLPs

Figure skating scoring is challenging because it requires judging the technical moves of the players as well as their coordination with the background music. Most learning-based methods cannot solve it well for two reasons: 1) each move in figure skating changes quickly, hence simply applying traditional frame sampling will lose a lot of valuable information, especially in 3 to 5 minutes long videos; 2) prior methods rarely considered the critical audio-visual relationship in their models. Due to these reasons, we introduce a novel architecture, named Skating-Mixer. It extends the MLP framework into a multimodal fashion and effectively learns long-term representations through our designed memory recurrent unit (MRU). Aside from the model, we collected a high-quality audio-visual FS1000 dataset, which contains over 1000 videos on 8 types of programs with 7 different rating metrics, overtaking other datasets in both quantity and diversity. Experiments show the proposed method achieves SOTAs over all major metrics on the public Fis-V and our FS1000 dataset. In addition, we include an analysis applying our method to the recent competitions in Beijing 2022 Winter Olympic Games, proving our method has strong applicability.

==> LaTeX/Section/01_Introduction/manuscript.tex <==
% \begin{center}
%     \begin{overpic}[width=1.0\linewidth]{}
%     \end{overpic}
%   \captionsetup{type=figure}
%     \captionof{figure}{\textbf{\textbf{Pipeline of Skating-Mixer.}} We adopt patch modeling methods just like \cite{dosovitskiy2020image, tolstikhin2021mlp}, and use TimeSformer~\cite{bertasius2021spacetime} and AST~\cite{gong2021ast} as our projection backbones. The memory unit of Skating-Mixer works for the recurrent mechanism. After integral learning in both spatial and temporal information, Skating-Mixer obtains a representation of long-range video. We integrate the outputs from each Skating-Mixer block into a head module and finish the figure skating scoring. \texttt{[MEM]} denotes the memory token and \texttt{[CLS]} denotes the class token.
%     }
% \label{fig:pipeline}
%   \end{center}
  
\begin{figure*}[h]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=0.75 \linewidth]{LaTeX/image/framework1.pdf}
\end{center}
\vspace{-10pt}
    \caption{\textbf{\textbf{Pipeline of Skating-Mixer.}} We utilize patch modeling methods just like \cite{dosovitskiy2020image,tolstikhin2021mlp}, and use TimeSformer~\cite{bertasius2021spacetime} and AST~\cite{gong2021ast} as our projection backbones. 
    %The memory recurrent unit (MRU) of Skating-Mixer works for the recurrent mechanism.
    The memory recurrent unit (MRU) of Skating-Mixer works for learning sequential temporal multimodal information.    
    %
    After integral learning in both spatial and temporal information, Skating-Mixer obtains a representation of long-range video. 
    % We integrate the outputs from each Skating-Mixer block into a head module and finish the figure skating scoring. 
    We integrate the output of the CLS Mixer and the output of \texttt{[MEM]} from the last clip to finish the scoring.
    \texttt{[MEM]} denotes the memory token and \texttt{[CLS]} denotes the class token.}
\label{fig:pipeline}
\vspace{-10pt}
\end{figure*}

Due to the importance of fair competition, many worldwide sports committees devote themselves to regularizing the behaviors of both athletes and referees. 
As a supplementary tool, crowd workers seek to employ objective machine intelligence to judge the performances in competitions. Therefore, many learning-based assessment models~\cite{pirsiavash2014assessing,parmar2017learning,pan2019action,jain2020action,xiang2018s3d,li2018end} have been introduced in recent years.
% Nevertheless, few works proposed to score figure skating videos because of several key challenges:
\jf{However, few works proposed to score figure skating videos due to several key challenges:}


\begin{itemize}
    \item[$\bullet$]  
    %Additionally, the actions in figure skating videos usually change rapidly, so there is much more important fine-grained action information, which leads to a much larger amount of input data than general videos.
    \textbf{Requiring strong video representation learning.}
    (1) Figure skating videos are 3$-$5 minutes long and contain manifold technical movements, requiring effective representation learning on the long videos with large fps (frame per second) \jf{which results in large size of inputs.} (2) Both audio and video should be considered when calculating the scores in figure skating.
    \item[$\bullet$] 
    %Different from videos in general scenarios that are collected from social networks and v-portal, the figure skating videos are captured from real sports competitions, which requires large amounts of human effort.
    
    \textbf{Missing high-quality dataset. }
    %Unlike common videos collected from social media and video portals, 
    Unlike common videos,
    figure skating videos are sourced from live sporting tournaments that require extensive manual process effort. This could be the reason that existing datasets~\cite{xu2019learning,liu2020fsd} are not comprehensive enough (in scale or diversity) to cover figure skating.  
\end{itemize}


To solve the first challenge, earlier work~\cite{liu2020fsd} utilized a hierarchical LSTM model to capture the local and global information in figure skating videos. The recent Eagle-eye method~\cite{nekoui2021eagle} considers pose heatmaps and appearance features jointly. Although these two methods achieve comparably good results, they remain obvious deficiencies. 
% Firstly, their architecture is fairly complex: they contain several streams with multiple well-designed CNN or LSTM blocks.
Firstly, their methods can hardly generalize to different categories of competitions in the real scene.
More importantly, they merely consider visual modality. %\mc{We argue that a}lthough technical action is an essential part of figure skating, background music should not be ignored in the scoring system. 
While technical action (visual modality) is important in figure skating, we argue that background music (audio modality) should not be ignored as well.
%Therefore, we argue that an efficient model which considers both visual and audio cues is urgently needed in this field.
An efficient model which considers both visual and audio cues is urgently needed in this field.

Convolutional Neural Networks~\cite{cnn} have long been used for various computer vision tasks~\cite{zhuge2022cubenet}. With the success in Natural Language Processing, Transformers~\cite{vaswani2017attention} have been introduced into the computer vision area and show great power in multimodal learning compared with CNNs~\cite{zhuge2021kaleido}. However, the complexity of Vision Transformer~\cite{dosovitskiy2020image} is quadratic in the
number of input patches and it usually requires a large amount of data to train~\cite{Liu2021EfficientTO}, which is hardly satisfied in our specific task. Recently, a pure MLP-based structure MLP-Mixer has been proposed and shows promising results on the image classification task~\cite{tolstikhin2021mlp} with linear complexity. Yet, this simple structure has not been deeply explored in the audio-visual area.
%Therefore, we introduce Skating-Mixer, which is the first MLP-based multimodal architecture and the first to learn the audio and visual information from figure skating videos.
Therefore, we introduce Skating-Mixer, which is the pioneer of MLP-based multimodal architecture and also the first to %learn the audio and visual information from figure skating videos.
score figure skating with both auditory and visual feature.
Skating-Mixer has the following properties: $(1)$ It simultaneously models audio and visual features, and learns the long-term joint representation in an effective way; $(2)$ By using the memory recurrent unit (MRU), this approach accurately predicts the results using extremely long-range cues; $(3)$ %with the simple architecture, it could avoid gradient vanishing and exploding problem and performs outstandingly.
% \mc{With its simple design, it could avoid the gradient vanishing and exploding problems which may face with Transformer~\cite{vaswani2017attention,devlin2018bert} or LSTM~\cite{hochreiter1997long} architecture.}
With its simple design, it could avoid the gradient vanishing and exploding problems in the vanilla recurrent neural network~\cite{rnn}.
%In this paper, we focus on discussing the figure skating scoring task due to our specific needing.
% \Rev{Apart from the advantages mentioned above}, our model can be used in many sport-related tasks, and even extend to general long-term scenarios.

Moreover, we observe that few high-quality datasets are set up for this task.
% Video data in FSD-10~\cite{liu2020fsd} and MCFS~\cite{DBLP:conf/aaai/LiuZLZXDZ21} are segmented into clips  action recognition task.
% Fis-V~\cite{xu2019learning} contains the complete videos for scoring, but it only contains ladies short program videos.
Fis-V~\cite{xu2019learning} only contains ladies short program videos.
%We find that just using visual features is enough to score such monotonous data.
Since the data distribution is monotonous, this dataset is less challenging.
In this case, we build a new dataset FS1000 with more than 1000 videos, 8 categories of figure skating, and 7 detailed scores to increase the diversity and quantity. The dataset requires the model to learn the underlying features across different figure skating videos.
Experiments conducted on both datasets demonstrate that Skating-Mixer not only achieves state-of-the-art results %but also shows the potential generalization over all types of figure skating with multimodality.
but also has the ability to generalize to all sorts of figure skating, making a good example  to tackle multimodal representation in sports.
% To validate the effectiveness of our method, we conducted experiments on the Fis-V dataset and our proposed FS1000 datasets, and demonstrate that our method not only achieves state-of-the-art results in figure skating but also shows the potential generalization in figure skating fields. 
% The followings are the primary contributions of this paper:
In summary, the primary contributions of this paper are listed as following:
\begin{itemize}
    \item[$\bullet$]  
    %we present a novel multimodal MLP-based framework to introduce both acoustic and visual modality in end-to-end figure skating scoring for the first time,
    %We provide a novel (and maybe the first) multimodal MLP-based framework that incorporates both audio and visual modalities in end-to-end figure skating scoring.
    \vspace{-3pt}
    We present the pioneer MLP-based multimodal framework that can model extremely long-range videos. It automatically scores figure skating with both auditory and visual information.
    \vspace{-3pt}
    \item[$\bullet$]  
    %we collect an elaborated FS1000 dataset, including, more long-range videos that contain all types of figure skating with more detailed scores,
    We collect a comprehensive FS1000 dataset, including more long-range videos that contain all types of figure skating with more detailed score records.
    \vspace{-2pt}    
    \item[$\bullet$]  
    We benchmark recent methods in this field on both Fis-V and FS1000 datasets.
    The proposed MLP-based and framework outperforms other CNN-based~\cite{parmar2017learning, parmar2019action}, LSTM-based~\cite{xu2019learning}, and Transformer-based~\cite{lee2020parameter} methods.
\end{itemize}
% \vspace{-3pt}

==> LaTeX/Section/02_RelatedWork/manuscript.tex <==
% We first review current technologies deployed in audio-visual learning. Then, we discuss previous MLP-based models and some researches in learning to score figure skating videos.

% \vspace{-10pt}
\subsection{Audio-Visual Learning}
There exists a rich exploration in audio-visual multimodal learning, especially in the deep learning era~\cite{zhu2021deep}. 
And datasets~\cite{chen2020vggsound,lee2021acav100m,gemmeke2017audio,abu2016youtube} involving representation learning in this field have been also developed.
%
%Subsequent to 
% Along with the success of these work, tasks including location~\cite{lathoud2004av16}, recognition~\cite{liu1997audio}, matching~\cite{nagrani2018learnable} and generation~\cite{wan2019towards,wiles2018x2face} further reveal the powerful  capabilities of deep learning.
%
% In recent years, pre-training technologies~\cite{devlin2018bert,zhuge2021kaleido} have become the main solutions to visual-audio issues.
%
M-BERT~\cite{lee2020parameter} focuses on reducing the complexity when introducing Transformer into audio-visual representation learning.
% , which inspires us to design a more efficient model in the field. 
% And VATT~\cite{akbari2021vatt} and VX2TEXT~\cite{lin2021vx2text} further propose universal multimodal transformer architectures bridging video, audio and text.
%
AVAS~\cite{morgado2020learning} attempts to learn the spatial alignment between audio and vision by introducing a new self-supervised proxy task.
%
Besides, another work~\cite{nagrani2021attention} also proposes to design a middle bottleneck to integrate audio and video modalities.
%
Although many existing methods explore audio-visual learning by various techniques, our proposed Skating-Mixer is the first attempt to apply MLP architecture to tackle this problem.

% \vspace{-10pt}
\subsection{MLP-based Architecture}
Attention-based network Transformer~\cite{vaswani2017attention,ji2022masked} achieve unparalleled success in NLP field, while convolutional networks~\cite{He_2016_CVPR} are still the main solution for most vision tasks~\cite{zhuge2022salient} until the proposal of ViT~\cite{dosovitskiy2020image}. 
Recently, MLP-Mixer~\cite{tolstikhin2021mlp} argue that MLP can be an alternative solution for vision representation learning.
% Besides, gMLP~\cite{liu2021pay} also demonstrates that all-MLP architecture can achieve competitive performances on both vision and NLP tasks. 
% Subsequently, many MLP-based architectures~\cite{yu2021s,hou2021vision,lian2021mlp,chen2021cyclemlp,zheng2021rethinking,lee2021moi,tang2021sparse,lou2021sparse,ren2021cascaded} emerged in large numbers.
Subsequently, many MLP-based architectures emerged in computer vision area.
S$^2$-MLP~\cite{yu2021s} only contains channel-mixing MLP and utilizes a spatial-shift operation for communication among patches. 
% The Permutator~\cite{hou2021vision} encodes the feature representations along height and width dimensions separately and enables itself to capture long-range dependencies along different directions. 
% Inspired by axial attention~\cite{ho2019axial}, AS-MLP~\cite{lian2021mlp} and sMLP~\cite{tang2021sparse} propose to restrict the MLP layer's reception field to reduce the computational complexity. 
In addition, there are several specific-function models being proposed, such as CycleMLP~\cite{chen2021cyclemlp} used in dense prediction, MixerGAN~\cite{cazenavette2021mixergan} and CrossMLP~\cite{ren2021cascaded} in image translation, and Mixer-TTS~\cite{tatanov2021mixer} in the text-to-speech task. Distinguished from the aforementioned works, our proposed model is the first MLP model solving audio-visual problems.

% \vspace{-10pt}
\subsection{Figure Skating}
% Due to the long-term and multimodal characteristics of figure skating videos, it is still quite challenging to learn to score figure skating by applying deep learning models.
In the computer vision field, the earliest work about figure skating can be traced back to MIT-Skating~\cite{pirsiavash2014assessing}, which gathered Olympic videos and assessed the actions. 
Similar research~\cite{xu2019learning} also focuses on scoring figure skating videos and collects a Fis-V dataset with 500 videos. 
However, Fis-V dataset only considers ladies single program, making it hard for generalization in this field. 
\cite{liu2020fsd} introduces action recognition in figure skating and meanwhile designs an FSD-10 dataset. 
% This dataset splits the complete competition video into several clips, therefore it is more suitable for fine-grained learning rather than studying the whole representation. 
% \Rev{MCFS dataset~\cite{DBLP:conf/aaai/LiuZLZXDZ21} consists of 271 samples and is fine-grained semantic, specialized and motion-centered. 
Another fine-grained, motion-centered MCFS dataset~\cite{DBLP:conf/aaai/LiuZLZXDZ21} is  proposed for the temporal action segmentation task. 
% Additionally, several researches~\cite{nakano2020estimating,zeng2020hybrid,nekoui2021eagle} propose dedicated models in figure skating area.
Additionally, several dedicated models have been proposed.
% Specifically, 1D CNN~\cite{nakano2020estimating} draws on a physiological reaction that people naturally suppress blinks during attention-grabbing moments, to detect the highlight in figure skating programs. 
Specifically, \cite{nakano2020estimating} detects the highlight in figure skating programs with people's reaction.
ACTION-Net~\cite{zeng2020hybrid} strengthens the importance of postures in long videos, learning both context and temporal discriminative information. 
% Considering joints and appearance dynamics are also key for performance improvement.
EAGLE-Eye~\cite{nekoui2021eagle} creates a two-stream pipeline to learn the long-term representation of figure skating actions. 
Compared with the others, our model is the first attempt to solve figure skating scenarios using both audio and video cues.

==> LaTeX/Section/03_Dataset/annotation.tex <==
\vspace{-5pt}
\subsection{Annotation and statistics}
{\bf Annotation.} As mentioned above, there are totally eight categories of figure skating competitions, namely, men/ladies/pairs short program (\textbf{MS}, \textbf{LS}, \textbf{PS}), men/ladies/pairs free skating (\textbf{MF}, \textbf{LF}, \textbf{PF}) and ice dance rhythm dance/free dance (\textbf{IR}, \textbf{IF}). 
%We labeled each video with its corresponding category and carefully annotated it with authorized scores.
We carefully labeled each video with its official scores according to the referee reports, and also player ID and corresponding category. 
In the scoring regulation of figure skating, the result can be divided into two parts: Technical Element Score (\textbf{\emph{TES}}) and Program Component Score (\textbf{\emph{PCS}}).
\textbf{\emph{TES}} evaluates the difficulty and execution of all technical movements, and \textbf{\emph{PCS}} describes the overall performance, considering five aspects: the Skating Skills  (\textbf{\emph{SS}}), Transitions  (\textbf{\emph{TR}}), Performance  (\textbf{\emph{PE}}), Composition  (\textbf{\emph{CO}}), and Interpretation of music (\textbf{\emph{IN}}).
Specifically, the Skating Skills assesses the skater's command of the blade over the ice; Transitions evaluates skaters' ability to transit between technical elements naturally; Performance shows the appeal and personality of the program; Composition reflects the choreography and the purpose to the way the program is constructed, and Interpretation is more concerned with the consistency between each movement and a corresponding beat in music.
Besides, there is a factor that indicates different weights of \textbf{\emph{PCS}} scores in different competitions.
These scores are given by nine different professional referees and calculated by the referee rules of figure skating competition.
Each video in the FS1000 dataset is annotated with these information mentioned above. 

\vspace{-2pt}
\noindent{\bf Statistics.} 
There are totally 1604 figure skating videos in our FS1000 dataset: 1247 videos are for training and validation while 357 videos from contests in 2022 are for testing, including Beijing 2022 Olympics.
Each video has $\sim$5000 frames with a frame rate of 25 and is annotated with detailed ground-truth scores.
Some example frames and the percentage of the number of each category in the FS1000 dataset are shown in Figure~\ref{fig:dataset_example}(a). 
As the videos contain complete snippets of each performance, they are relatively long with a duration ranging from 2.5 minutes to 4.3 minutes, and the average duration of all videos is about 3 minutes and 20 seconds.
The details of each category's average length are given in Figure~\ref{fig:dataset_example}(b).
We can see that compared with the duration of short program and rhythm dance (2 to 3 minutes), free skating and free dance generally have a longer duration (about 4 minutes), which is consistent with the standards of different competitions.
% Furthermore, we also conduct some statistical analysis. In particular, we calculate the average TES and PCS scores over different types of matches shown at the bottom of Figure~\ref{fig:duration and scores}. 
% For each category, skaters usually obtain a slightly higher TES scores than PCS scores except for men and pairs free skating matches.
% And since there are some differences in the scoring criteria between free skating and short program, the average scores of different matches may looks quite different.
% Furthermore, we calculate the average \textbf{\emph{TES}} and \textbf{\emph{PCS}} scores over different types of program shown at the bottom of Figure~\ref{fig:dataset_example}(c). Since there are some differences in the scoring criteria between free skating and short program, the average scores between them may look quite different.
%And the Spearman correlations among five scores included in \mc{\textbf{\emph{PCS}}} are also computed as shown in Figure~\ref{fig:heatmap}. These correlation values in the heatmap reflect that although these five scores represent different meanings, they are actually highly correlated with each other. %Because of this, it is possible to predict these scores in one single model. 
% \mc{So it makes sense to predict these scores with a single model.}

% \begin{figure}[t]
% \begin{center}
% % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=0.9\linewidth]{latex/image/average_duration.pdf}
% \end{center}
%   \caption{Average duration of figure skating videos per category.}
% \label{fig:average_duration}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=0.9\linewidth]{latex/image/average_score.pdf}
% \end{center}
%   \caption{Average scores players got in each type of figure skating competitions.}
% \label{fig:average_score}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=0.9\linewidth]{latex/image/duration and scores.pdf}
% \end{center}
% \vspace{-15pt}
%   \caption{Average scores players got in each type of figure skating competitions and average duration of figure skating videos per category.}
% \label{fig:duration and scores}
% \vspace{-15pt}
% \end{figure}



% comparison with existing datasets of figure skating.

==> LaTeX/Section/03_Dataset/comparison.tex <==
\vspace{-4pt}
\subsection{Comparison with other datasets}
\vspace{-7pt}
\begin{table}[h!]
%\normalem
	\renewcommand\tabcolsep{4.0pt}
	\centering
	\scalebox{0.75}{
        \begin{tabular}{l|c|c|c|c|c|c}
        \toprule
\rowcolor{blue!10}
        \textbf{Dataset} &\textbf{Task} & \bf $\#$ Video & \bf Length  & \bf $\#$ Score & \bf $\#$ Type & \bf Feature \\  \hline
        FSD-10 & AR & 1484 & ~10h & 1 & - & V    \\
        MCFS & AS & 271 & ~5h & - & - & V    \\ \hline
        MIT-Skate & LS & 171 & 8h  & 1  & 1 & V  \\ 
        FisV & LS & 500 & 24h & 2 & 1 & V  \\
        
        FS1000 (ours) & LS & 1604 & 91h &  7 & 8 & A+V  \\  
        \bottomrule   
        \end{tabular}
    }
\caption{Dataset comparison in figure skating area. Length refers to the total length of all videos. (AR: Action Recognition, AS: Action Segmentation, LS: Long-video Scoring.)}
\vspace{-10pt}
\label{tab: dataset}
\end{table}
\noindent Here, we show the comparison between our proposed FS1000 dataset and other existing figure skating video datasets: MCFS~\cite{DBLP:conf/aaai/LiuZLZXDZ21}, FSD-10~\cite{liu2020fsd}, FisV~\cite{xu2019learning} and MIT-Skate dataset~\cite{pirsiavash2014assessing, parmar2017learning}. 
% For the MIT-Skate dataset, we demonstrate the extended version mentioned in~\cite{parmar2017learning}.
% The comparison between these datasets is shown in Table~\ref{tab: dataset}.
% It includes the target task, video number, video duration and the number of annotated scores and figure skating types. 
FSD-10 and MCFS focus on the technical actions in figure skating and they only contain short clips of each action instead of the complete videos, which is not suitable for our multimodal scoring task. 
% They both segment the whole video into clips with certain actions.
% FSD-10 annotates each clip with a single score for each action, which differs from the scores of whole program in our dataset. 
% These two datasets are designed for action-related tasks so they only contain small clips of each action instead of the complete videos. So they are not suitable for our task.
% Note that FSD-10 just annotates each clip with  the execution score for each while TES is a total score for all the actions.
MIT-Skate, Fis-V and our proposed FS1000 are all set up for long-video scoring tasks. MIT-Skate consists of videos that happened before 2012, which is outdated because of the regulation change. 
Also, it only contains 171 ladies short program videos, which is too limited in scale. 
Therefore, we focus on the last two datasets in our work. 
We can see that our dataset is the first one to utilize audio feature in this area and overtakes the other datasets in quantity and diversity.
% \vspace{-10pt}
% \begin{table}[h!]
% %\normalem
% 	\renewcommand\tabcolsep{4.0pt}
% 	\centering
% 	\scalebox{0.75}{
%         \begin{tabular}{l|c|c|c|c|c|c}
%         \toprule
% \rowcolor{blue!10}
%         \textbf{Dataset} &\textbf{Task} & \bf $\#$ Video & \bf Length  & \bf $\#$ Score & \bf $\#$ Type & \bf Feature \\  \hline
%         FSD-10 & AR & 1484 & ~10h & 1 & - & V    \\
%         MCFS & AS & 271 & ~5h & - & - & V    \\ \hline
%         MIT-Skate & LS & 8h & 150s  & 1  & 1 & V  \\ 
%         FisV & LS & 500 & 23h & 2 & 1 & V  \\
        
%         FS1000 (ours) & LS & 1605 & 91h &  7 & 8 & A+V  \\  
%         \bottomrule   
%         \end{tabular}
%     }
% \caption{Dataset comparison in figure skating area. (AR: Action Recognition, AS: Action Segmentation, LS: Long-video Scoring.)}
% \vspace{-20pt}
% \label{tab: dataset}
% \end{table}

==> LaTeX/Section/03_Dataset/data_collection.tex <==
\subsection{Data Collection}
% \subsubsection{Data Source.}
\noindent\textbf{Data Source.}
% {\bf Data Source.} %With an aim to obtain a great quantity of figure skating videos with both high visual and audio quality, we carefully select and download videos only from the highest level of international skating competitions with standard and fair judgment. 
%
With an aim to obtain high-quality figure skating videos, we carefully selected and downloaded videos only from the top-tier international skating competitions.
% with standard and fair judgment.
%Besides, we also collect authorized scores to annotate our dataset. 
Besides, we also collected and checked scores from referee reports to annotate our dataset in authoritative.\footnote{https://www.isu.org/figure-skating/entries-results/fsk-results}
%
Specifically, ISU World Figure Skating Championships, ISU Grand Prix of Figure Skating, \emph{etc.,} %are selected as our source videos. 
are selected as our main data sources.
%Normally, figure skating consists of four primary categories, namely, men's singles, ladies' singles, pair skating and ice dance.
Normally, figure skating consists of 4 primary categories: mens singles, ladies singles, pair skating and ice dance.
% Noted that the latter two are both performed by couples, and pair skating focuses more on technical move while ice dance values more on the artistic component in the performance.
Each primary category contains short program and free skating (in ice dance, they are called rhythm dance and free dance). So, there are 8 subdivided categories, as shown in Figure \ref{fig:dataset_example}.

% In the short program, players are required to perform fixed technical actions to show their basic skills while free skating provides more freedom and allows complex actions and better expression for background music.
% In order to maintain data diversity and fully extract the correlations between players' performances (video-modality) and music (audio-modality), %thus all these four kinds of competitions are collected to construct our FS1000 dataset.  
% all types of program have been organized to construct our FS1000 dataset.  
% Note that since the % mark scheme keeps slightly changing every year, we only utilized the competition videos that happened in 2018 and 2019 in our figure skating video dataset to make the scores more comparable.
% referee rules keep slightly changing every year, we utilized the competition videos that happened in recent four years in our figure skating video dataset to make the scores more comparable.

\noindent{{\bf Pre-processing.}}
% {\bf Pre-processing.}
% \subsubsection{Pre-processing.}
%Each video of figure skating competitions are usually untrimmed, ranging from $1$ hour to $5$ hours and consisting of the performances of all participants as well as highlight replay, warming up parts.
The raw videos collected from figure skating competitions are usually untrimmed and record the whole procedure ranging from $1$ to $5$ hours. It consists of the performances of all players as well as highlight replay, warming up parts, and waiting for score parts. 
These redundant contents are usually not helpful for score judgment.
We initially downloaded over {$400$-hour} videos and then
% different from previous figure skating datasets that contain those redundant parts, we
manually processed all videos, only reserving pure competition performance clips of players from the exact beginning to the ending moment of background music. 
%This important pre-processing step \mc{takes more than 60 video editing},
% Five professional people participate in video editing and takes nearly 2 months to finish this important pre-processing step.
% This time-consuming pre-processing ensures each video sample can exactly cover the intactness of player's performance. %correspond to its ground-truth scores. 
% Additionally, %some poor-quality videos that are not fluent and very blurred without audio were removed to maintain the high standard of FS1000 dataset.
% poor-quality videos that are not fluent, blurred, or without audio, were removed to maintain the high standard of FS1000 dataset.

==> LaTeX/Section/03_Dataset/manuscript.tex <==
\begin{figure*}[h]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \vspace*{-25pt}
\includegraphics[width=0.9\linewidth]{LaTeX/image/data_aaai1.pdf}
\end{center}
\vspace{-15pt}
    \caption{%Example video frames and the percentage of each category
    The distribution, average length, and video samples for each category in FS1000. \textbf{{MS}:} men short program \emph{(16\%)}, \textbf{{MF}:} men free skating \emph{(13\%)}, \textbf{{LS}:} ladies short program \emph{(19\%)}, \textbf{{LF}:} ladies free skating \emph{(13\%)}, \textbf{{PS}:} pairs short program \emph{(8\%)}, \textbf{{PF}:} pairs free skating \emph{(9\%)}, \textbf{{IF}:} ice dance free skating \emph{(9\%)}, and \textbf{{IR}:} ice dance rhythm dance \emph{(13\%)}.}
\label{fig:dataset_example}
\vspace{-15pt}
\end{figure*}
To further facilitate the research of learning-based figure skating scoring, we present the largest figure skating dataset FS1000 with high-quality videos.
%All video clips come from high-standard international figure skating competitions and were captured by professional camera devices.
All videos come from high-standard international figure skating competitions and were captured by professional camera devices.
% The dataset is designed for several downstream tasks, including learning to predict scores of participants in each group and recognize the category of each competition.
The dataset is designed for predicting scores in figure skating competitions, with rich annotations like player ID and program categories, which may facilitate this field even more. %, such as video understanding, classification or motion recognition.

\input{Section/03_Dataset/data_collection}

% \vspace{-15pt}
\input{Section/03_Dataset/annotation}

\input{Section/03_Dataset/comparison}

==> LaTeX/Section/04_Method/attentive_mlpmixer.tex <==
\subsubsection{Attentive MLP-Mixer.}
\begin{figure}[h]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \vspace*{-25pt}
\includegraphics[width=1.0\linewidth]{LaTeX/image/att_mlp.pdf}
\end{center}
% \vspace*{-15pt}
    \caption{%Example video frames and the percentage of each category
    Structure comparison between the original MLP-Mixer and the Attentive MLP-Mixer.}
\label{fig:att_mlp}
% \vspace{-20pt}
\end{figure}
After processing all the clips in the video, we could directly use the final memory token output for scoring. However, we still want the model could utilize more local information in each clip and have an exhaustive understanding on such long sequence.
In figure skating, every clip does not contribute equally to the final score. Some technical moves or falls can significantly affect the final result.
One solution is to collect all the $\texttt{[CLS]}$ tokens and input those tokens with position embeddings to another MLP-Mixer block. Directly using MLP-Mixer could implicitly find the important part of the performance. 
Additionally, we propose a new structure, Attentive MLP-Mixer, which explicitly allows our model focus more on the important clips. Unlike the original MLP-Mixer block which first mixes token feature and then mixes channel feature, our structure first input the tokens into channel-mixing MLP and utilize sigmoid activation function to obtain token weights. The weights are multiplied with the original feature input. After that, the resulted tokens are input into the token-mixing MLP for further results.
To be more specific, suppose $\mathbf{C}$ is the concatenated tokens:
\begin{equation}
    \mathbf{C} = [\texttt{CLS}_1 \texttt{CLS}_2 ... \texttt{CLS}_t]
\end{equation}
The attention MLP-Mixer could be described as follow:
\begin{equation}
    \begin{aligned}
    \mathbf{X} &= \mathbf{C} + PE_c\\
    \mathbf{Z}_{j, *}&=\mathbf{X}_{j, *}+\mathbf{W}_{2} \Phi \left(\mathbf{W}_{1} \text{Norm}(\mathbf{X}_{j, *})\right),\\
    \mathbf{U} &= \sigma(\mathbf{Z}) \odot \mathbf{C} \\
\mathbf{Y}_{*, i}&=\mathbf{U}_{*, i}+\mathbf{W}_{4} \Phi \left(\mathbf{W}_{3} \text{Norm}(\mathbf{U}_{*, i})\right),
    \end{aligned}
\end{equation}
where $\odot$ denotes the element-wise production. The structure is shown in Figure~\ref{fig:att_mlp}. We took the mean value of the resulted features and concatenate with the last memory token output. The final score is generated by a linear layer. 

==> LaTeX/Section/04_Method/manuscript.tex <==
%In this section, we introduce our MLP-based model. %for figure skating scoring.
% In this section, we comprehensively introduce our MLP-based multimodal model, the \textbf{Skating-Mixer}. %for figure skating scoring.
%We consider both acoustic and visual features as input in this method. %the scoring system. 
%Due to the lack of a large amount of data in figure skating area, complicated models easily get over-fitted in related tasks.
%In this case, %an MLP-Mixer-based model is simple but efficient.
%our simple but efficient Skating-Mixer model is proposed.
% The fundamental architecture is made up of Mixer layers~\cite{tolstikhin2021mlp}. It is simple enough to avoid intricate designs, while yet surpassing CNN-based~\cite{parmar2019action}, LSTM-based~\cite{xu2019learning}, and Transformer-based~\cite{lee2020parameter} architectures.
% The pipeline is shown in Figure~\ref{fig:pipeline}.

% \input{Section/04_Method/mlpmixer}

% \input{Section/04_Method/recurrent_mlp}
\input{LaTeX/Section/04_Method/newstructure}

==> LaTeX/Section/04_Method/mlpmixer.tex <==
% \vspace{-10pt}
\subsection{Preliminary: MLP-Mixer}
% \subsubsection{MLP-Mixer}

In~\cite{tolstikhin2021mlp}, an MLP-based architecture has been proposed in the computer vision area and shows that %exclusively multi-layer perceptrons are powerful enough to achieve excellent results on image classification tasks.
model organizing multi-layer perceptrons are powerful enough to achieve excellent results on image classification tasks.
Similar to Visual Transformer~\cite{dosovitskiy2020image}, input images for MLP-Mixer~\cite{tolstikhin2021mlp} are split into several non-overlapping patches and each patch is treated as a sequence token. 
MLP-Mixer contains several identical layers, and each layer contains two MLP blocks: channel-mixing MLP and token-mixing MLP. 
Channel-mixing MLP operates on the channel dimension of the input feature, allowing different channels to communicate with each other; token-mixing MLP operates on the token dimension, so information could flow across different tokens and communicate with each other. 
Each block contains two MLP layers, and one GELU~\cite{hendrycks2020gaussian} activation function (described as $\Phi$). Besides, skip connection is also applied in each block. 

To be more specific, suppose $\mathbf{X} \in \mathbb{R}^{S \times C}$ is a two-dimension input feature, where $S$ is the sequence length (number of tokens) and $C$ is the number of channels for each token. In each layer, the function could be represented as:
\begin{equation}
\begin{aligned}
\mathbf{U}_{*, i}&=\mathbf{X}_{*, i}+\mathbf{W}_{2} \Phi \left(\mathbf{W}_{1} \text{Norm}(\mathbf{X}_{*, i})\right),\\
% , & \text { for } i=1 \ldots C \\
\mathbf{Y}_{j, *}&=\mathbf{U}_{j, *}+\mathbf{W}_{4} \Phi \left(\mathbf{W}_{3} \text{Norm}(\mathbf{U}_{j, *})\right),
% , & \text { for } j=1 \ldots S
\end{aligned}
\label{MLP-Mixer}
\end{equation}
where $i$ ranges from $1 \ldots C$, and $j$ ranges from $1 \ldots S$. 
$\text{Norm}$ denotes LayerNorm~\cite{ba2016layer} and $\mathbf{W}$ represents the weights of linear layer in each block. Input feature first passes through token-mixing MLP and then follows channel-mixing MLP.
% According to the author, it is unnecessary to use position encoding since token-mixing MLP is able to detect the order of input tokens.
This structure allows each element in the input feature could interact with other features along two dimensions.

==> LaTeX/Section/04_Method/newstructure.tex <==
% \subsection{Skating Mixer}
% Figure skating videos usually last minutes and require large fps to identify each action, which results in a gigantic input video visual feature.
In this section, we comprehensively introduce our MLP-based multimodal model, the \textbf{Skating-Mixer}.
In our task, the model should be capable of handling extremely long videos with large fps, which means gigantic input audio-visual feature.
\jf{Models like ViT~\cite{dosovitskiy2020image} can hardly handle these data due to the memory limit.}
Unlike previous methods~\cite{bain2021frozen,lei2021less} that sample several frames to represent a whole video, we segment the video into multiple 5-second clips and input them to projection models~\cite{gong2021ast,bertasius2021spacetime} to obtain audio and video features respectively. 
This is because our model needs to deal with both audio and visual features and sampling frames will cause these two features unaligned.
\jf{Also, sampling frames will lose information of fast motions.}
The whole framework is shown in Figure~\ref{fig:pipeline}.
Suppose there are $T$ clips in the video.
For the $t$-th clip in the video, $\textbf{A}_t$ and $\textbf{V}_t$ denote the input audio feature and video feature, respectively.

\vspace{-5pt}
\subsubsection{Memory Recurrent Unit.}
\begin{figure}[h]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \vspace*{-25pt}
\includegraphics[width=0.9\linewidth]{LaTeX/image/newstruct3.pdf}
\end{center}
\vspace{-10pt}
    \caption{%Example video frames and the percentage of each category
    The structure of memory recurrent unit.}
\label{fig:newstruct}
\vspace{-10pt}
\end{figure}
The structure of memory recurrent unit (MRU) is shown in Figure~\ref{fig:newstruct}. This unit tends to capture the long-term relationships in the video and obtain a comprehensive overview of the whole video. 
The main idea of MRU is to split the video into several clips and process clip by clip. However, it is also necessary to let each clip acquire the information from the previous clips.
Therefore, a memory token \texttt{[MEM]} is applied with audio and video input. The memory token is a learnable randomly-initialized vector. At the $t$-th clip, the input memory $\texttt{[MEM]}_{t-1}$ is first passed into two bottleneck structures to extract audio and video-related features from the previous clips, denoted as $\textbf{A}_t^{prev}$ and $\textbf{V}_t^{prev}$. $\textbf{A}_t^{prev}$ and $\textbf{V}_t^{prev}$ are concatenated with the feature input $\textbf{A}_t$ and $\textbf{V}_t$. Position embeddings are added with the concatenated feature to identify the time order of the input tokens:
\begin{equation}
\begin{aligned}
    \tilde{\textbf{A}}_t = [\textbf{A}_t^{prev} \ \textbf{A}_t] + PE_a \\
    \tilde{\textbf{V}}_t = [\textbf{V}_t^{prev} \ \textbf{V}_t] + PE_v
\end{aligned}
\end{equation}
The audio and video features are passed through two separate MLP-Mixer blocks, Audio-Mixer and Video-Mixer. The two MLP-Mixer blocks here enable each modality to fuse information along the time dimension. 
The resulted audio and video features, $\hat{\textbf{A}}_t$ and $\hat{\textbf{V}}_t$, could capture the long-term feature from previous clips.
% The resulted audio and video features are concatenated together.
Then, we use the same strategy as visual Transformer~\cite{dosovitskiy2020image} by using a \texttt{[CLS]} token. 
% The purpose of \texttt{[CLS]} token is to get a feature to represent the whole clip and use for further scoring. 
\texttt{[CLS]} token is also a learnable vector concatenated with $\hat{\textbf{A}}_t$ and $\hat{\textbf{V}}_t$. The concatenated feature is then input to another MLP-Mixer block, Multimodal Mixer to mix information across different modalities. The output of \texttt{[CLS]} token, $\texttt{[CLS]}_t$ is used to represent the whole video clip with multimodal information. 
% The process could be describe as follow:
% \begin{equation}
% \begin{aligned}
%     O_t = MLP-Mixer([\texttt{CLS}\ \hat{A_t}\ \hat{V_t}]) \\
%     C_t = O_t[0]
% \end{aligned}
% \end{equation}
Finally, $\texttt{[CLS]}_t$ is concatenated with the input memory token $\texttt{[MEM]}_{t-1}$ and pass through another MLP-Mixer block, Memory-Mixer. 
In the Memory-Mixer, the current clip representation will interact with the memory token and update the memory content. The output at the position of $\texttt{[MEM]}_{t-1}$ is $\texttt{[MEM]}_{t}$, which is the input memory token for the next clip.
The memory output of the last clip $\texttt{[MEM]}_T$ will be used for scoring. 
Besides that, we also collect all the $\texttt{[CLS]}$ tokens output and add with position embeddings:
\begin{equation}
\begin{aligned}
    \tilde{\textbf{C}} & = [\texttt{CLS}_1 \ \texttt{CLS}_2 \  ... \ \texttt{CLS}_T] + PE_c 
    % \vspace{-15pt}
\end{aligned}
\end{equation}
$\tilde{\textbf{C}}$ is then input to another Mixer block, CLS Mixer.
This block helps the model further learn the local information from each clip. The outputs of CLS Mixer are averaged and concatenated with $\texttt{[MEM]}_T$. The final score is generated by these two features with a linear layer.
% \begin{equation*}
%     \begin{aligned}
%     S = W([]) + b
%     \end{aligned}
% \end{equation*}
% where $W$ and $b$ are the parameters of linear layer. 

\noindent\textbf{Skating Mixer \emph{vs} LSTM.}
% \subsubsection{Skating Mixer \emph{vs} LSTM.}
The recurrent mechanism is similar to RNN~\cite{rnn} and LSTM~\cite{hochreiter1997long}, but the design of MLP-Mixer is simpler and is capable of dealing with multimodal data. In vanilla RNN architecture, when the input sequence becomes longer, gradient vanishing and gradient exploding happen.
% which will deteriorate the training of model.
In LSTM, this problem is solved by adding gate strategy. These gates control the information flow from the input to make the model focus on important parts of input and thus reduces the effective input length. In our architecture, it is not necessary to have delicately designed gates. Gradient vanishing and exploding issues could be mitigated since there is skip-connection within MLP-Mixer blocks and no extra projection is implemented for the memory token. Additionally, the proposed structure is capable of dealing with multimodal information, which is not considered in LSTM.
% \textcolor{red}{Moreover, the memory token from previous clip mixed with feature token from the current clip and enable memory token to choose which part of the information is worthwhile to be remembered.}
Mixing the memory token will enable the current clip to see the previous information and thus generate a comprehensive view for the whole video.


% \noindent{\textbf{Bidirection Mixer.}}
\noindent\textbf{Bi-direction Mixer.}
% \textbf{Bi-direction Mixer.}
% \subsubsection{Bi-direction Mixer.}
In our model, we use a similar strategy as in bidirectional recurrent neural network~\cite{rnn}, that is to add a backward direction in the model to grasp a comprehensive view of the whole video. For the backward direction, the last clip of the video will be processed first, then the memory flows to the first clip. 
% The initial memory token and input class token are the same as the forward direction. 
% So for each clip, there will be two [\texttt{CLS}] token outputs: one is forward output $\textbf{O}_t^{forward}$, the other one is backward output $\textbf{O}_t^{backward}$. We simply take the average value to represent each clip:
% For both $\texttt{[CLS]}$ and $\texttt{[MEM]}$ output, we took the average value of forward and backward direction. 
The averaged value of $\texttt{[CLS]}$ outputs from forward and backward directions at each clip are input to CLS Mixer; the averaged $\texttt{[MEM]}$ output of the last clip in forward and backward directions will be used for scoring.
 
% \begin{equation}
%     \mathbf{O}_t = \frac{\textbf{O}_t^{forward} + \textbf{O}_t^{backward}}{2}.
% \end{equation}


==> LaTeX/Section/05_Experiment/ablation.tex <==
\subsection{Ablation studies}
\begin{table*}[t]
\scriptsize
\centering
% \setlength\tabcolsep{1.82pt}
% \resizebox{\textwidth}{15mm}{
% \renewcommand\arraystretch{0.8}
\scalebox{0.9}{
\begin{tabular}{lr|cccc|ccc|ccc}
\toprule
\rowcolor{blue!10}
\textbf{Factor} &
  \multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{\textbf{Component}} &
  \multicolumn{3}{c|}{\textbf{Modality}} &
%   \multicolumn{4}{c|}{\textbf{Dropout}} &
  \multicolumn{3}{c}{\textbf{Scoring token}} \\
\rowcolor{blue!10}
\multicolumn{2}{l|}{}    & Mixer & Mixer+MEM & MRU & MRU+Bi-D & A & V & A+V & \texttt{[CLS]} & \texttt{[MEM]} & \texttt{[CLS]}+\texttt{[MEM]}\\ 
% \multicolumn{2}{l|}{}    &  &  &  & \textcolor{green!100}{\checkmark} &  &  & \textcolor{green!100}{\checkmark} &  &  & \textcolor{green!100}{\checkmark} \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fis-V\\ \end{tabular}} &
  \textit{TES} &
  23.25 (0.55) &
  20.34 (0.66) &
  20.07 (0.66) &
  \bf 19.57 (0.68) &
  33.04 (0.49) &
  20.56 (0.67) &
  \bf 19.57 (0.68) &
  21.53 (0.66) &
  20.10 (0.67) &
  \bf 19.57 (0.68) 
 \\
 & \textit{PCS}   & 10.87 (0.73)  
 & 8.75 (0.79)
 & 8.23 (0.81)    
 & \bf 7.96 (0.82)     
 & 14.68 (0.67) 
 & 9.97 (0.76)
 & \bf 7.96 (0.82) 
 & 8.55 (0.81)
 & 8.10 (0.82)
 & \bf 7.96 (0.82)
 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}FS1000\\ (Ours)\end{tabular}} &
  \textit{TES} &
  93.65 (0.85) &
  90.80 (0.87) &
  85.71 (0.88) &
  \bf 81.24 (0.88) &
  94.94 (0.82) &
  82.59 (0.88) &
  \bf 81.24 (0.88) &
  83.16 (0.86)&
  88.78 (0.86)&
  \bf 81.24 (0.88)
  \\
 & \textit{PCS} & 13.81 (0.75) 
 & 10.96 (0.80) 
 & 10.44 (0.81)    
 & \bf 9.47 (0.82)   
 & 20.40 (0.55)
 & 10.92 (0.79) 
 & \bf 9.47 (0.82)  
 & 10.37 (0.81)
 & 10.71 (0.79)
 & \bf 9.47 (0.82) 
\\ \bottomrule
\end{tabular}
}
\vspace{-5pt}
\caption{Ablation studies on different components, modalities and scoring tokens. The value outside the brackets is MSE while inside is Spearman correlation.
% For component part, \textbf{B}: Baseline; \textbf{TA}: Token Aggregation; \textbf{MRU}: Memory Recurrent Unit; \textbf{Bi-D}: Bi-direction. Figure~\ref{fig:abl_structure} shows the detailed comparison.
}
\vspace{-10pt}
%. For the number of Layers experiments are conducted on 1, 2 and 3 Mixer Layers. For dropout rate, 0\%, 10\%, 20\% and 30\% are analyzed here.}
\label{fig:abl} \end{table*}

\begin{table}[h!]
\scriptsize
\centering
% \setlength\tabcolsep{1.82pt}
% \renewcommand\arraystretch{1.0}
\scalebox{0.9}{
\begin{tabular}{l|c|cccc}
\toprule
\rowcolor{blue!10}
  \multicolumn{1}{c|}{\textbf{Dataset}} &
  \multicolumn{1}{c|}{\textbf{Backbone}} &
  \multicolumn{1}{c}{\textbf{\textit{TES}}} &
  \multicolumn{1}{c}{\textbf{\textit{PCS}}} &
  \multicolumn{1}{c}{\textbf{\# Params}} &
  \multicolumn{1}{c}{\textbf{MACs}}\\ \hline
% \rowcolor{blue!10}
% \multicolumn{2}{l|}{}    & \textbf{C3D[]} & \textbf{TimeSformer[]} & \textbf{C3D[]} & \textbf{TimeSformer[]}  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fis-V\\ \end{tabular}} &
  Transformer & 25.60 (0.51)
  & 13.18 (0.68)
  & 20.48M
  & 35.55G
    \\
 & MLP-Mixer & \bf 19.57 (0.68) & \bf 7.96 (0.82) & \bf 14.32M & \bf 24.95G    \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}FS1000\\ (Ours)\end{tabular}} &
  Transformer & 108.68 (0.81)
     & 13.40 (0.76)
     & 20.48M
     & 48.92G
  \\
 & MLP-Mixer & \bf 81.24 (0.88) & \bf 9.47 (0.82) & \bf 14.32M  & \bf 34.36G 
\\ \bottomrule
\end{tabular}
}
% \vspace{5pt}
\caption{Comparison of Transformer and MLP-Mixer as backbone in our Skating Mixer. MACs means Multiply–Accumulate Operations.}
\vspace{-15pt}
%. For the number of Layers experiments are conducted on 1, 2 and 3 Mixer Layers. For dropout rate, 0\%, 10\%, 20\% and 30\% are analyzed here.}
\label{tab:backbone} \end{table}

% \noindent{\textbf{Different feature extractor.}}
We have conducted ablation experiments on both datasets. Here we analyze two major scores, \textbf{\emph{TES}} and \textbf{\emph{PCS}}.

\begin{figure}[t!]
\centering
\includegraphics[width=1.0\linewidth]{LaTeX/image/structs.pdf}
\vspace{-20pt}
\caption{Four of our designed fusion structures. 
% \textbf{B}: baseline. \textbf{TA}: Token Aggregation. \textbf{MRU}: memory recurrent unit. \textbf{Bi-D:} bi-direction. The final version of our method is simple and elegant, without no intricate designs, thanks to the inspirations we got from previous outstanding neural networks~\cite{hochreiter1997long, vaswani2017attention, devlin2018bert, tolstikhin2021mlp, sun2019videobert}.
}
\vspace{-15pt}
\label{fig:abl_structure}\end{figure}

\noindent{\textbf{Component.}}
% \textbf{Component.}
% \subsubsection{Components.}
We first examine the effectiveness of our designed memory recurrent unit (MRU) and bi-direction propagation through four different fusion model structures, as shown in Figure~\ref{fig:abl_structure}. The first one (\textbf{Mixer}) is to simply input all the audio and video features into a large MLP-Mixer model for fusion. 
% The predicted score is generated by the [\texttt{CLS}] token. 
% Then, we aggregate the audio and video feature from the same clip and input them to the Mixer model together with [\texttt{CLS}] token. This process is called token aggregation (\textbf{B+TA}). The average score generated by  [\texttt{CLS}] tokens from all the video clips is used to produce the final score. 
% We then optimize such process by introducing the memory recurrent unit (\textbf{B+TA+MRU}). 
We then optimize such process by introducing the memory recurrent flow with MLP-Mixer (\textbf{Mixer+MEM}).
Then, the vanilla MLP-Mixer is replaced by our proposed MRU (\textbf{MRU}).
Finally, the bi-directional mechanism is applied with our proposed MRU (\textbf{MRU+Bi-D}).
The result is shown in Table~\ref{fig:abl}. 
The model fails to learn the long-term relationship between audio and video modalities when directly inputting all the features into a single model. Introducing memory mechanism helps the model capture long-term information and our proposed MRU could further better fuse multimodal features within extremely long videos. 
% By slicing the long video into short video clips, the model is capable to capture audio-visual information.
% \jf{By slicing the long video into short video clips, the model is capable to establish audio-visual relation.}
Moreover, adding bi-direction flow could effectively enhance the understanding of long videos and improve the performance of the model.

% \begin{table*}[t]
% \scriptsize
% \centering
% % \setlength\tabcolsep{1.82pt}
% % \resizebox{\textwidth}{15mm}{
% % \renewcommand\arraystretch{0.8}
% \scalebox{0.9}{
% \begin{tabular}{lr|cccc|ccc|ccc}
% \toprule
% \rowcolor{blue!10}
% \textbf{Factor} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{4}{c|}{\textbf{Component}} &
%   \multicolumn{3}{c|}{\textbf{Modality}} &
% %   \multicolumn{4}{c|}{\textbf{Dropout}} &
%   \multicolumn{3}{c}{\textbf{Scoring token}} \\
% \rowcolor{blue!10}
% \multicolumn{2}{l|}{}    & Mixer & Mixer+MEM & MRU & MRU+Bi-D & A & V & A+V & \texttt{[CLS]} & \texttt{[MEM]} & \texttt{[CLS]}+\texttt{[MEM]}\\ 
% % \multicolumn{2}{l|}{}    &  &  &  & \textcolor{green!100}{\checkmark} &  &  & \textcolor{green!100}{\checkmark} &  &  & \textcolor{green!100}{\checkmark} \\ 
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fis-V\\ \end{tabular}} &
%   \textit{TES} &
%   23.25 (0.55) &
%   20.34 (0.66) &
%   20.07 (0.66) &
%   \bf 19.57 (0.68) &
%   33.04 (0.49) &
%   20.56 (0.67) &
%   \bf 19.57 (0.68) &
%   21.53 (0.66) &
%   20.10 (0.67) &
%   \bf 19.57 (0.68) 
%  \\
%  & \textit{PCS}   & 10.87 (0.73)  
%  & 8.75 (0.79)
%  & 8.23 (0.81)    
%  & \bf 7.96 (0.82)     
%  & 14.68 (0.67) 
%  & 9.97 (0.76)
%  & \bf 7.96 (0.82) 
%  & 8.55 (0.81)
%  & 8.10 (0.82)
%  & \bf 7.96 (0.82)
%  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}FS1000\\ (Ours)\end{tabular}} &
%   \textit{TES} &
%   93.65 (0.85) &
%   90.80 (0.87) &
%   85.71 (0.88) &
%   \bf 81.24 (0.88) &
%   94.94 (0.82) &
%   82.59 (0.88) &
%   \bf 81.24 (0.88) &
%   83.16 (0.86)&
%   88.78 (0.86)&
%   \bf 81.24 (0.88)
%   \\
%  & \textit{PCS} & 13.81 (0.75) 
%  & 10.96 (0.80) 
%  & 10.44 (0.81)    
%  & \bf 9.47 (0.82)   
%  & 20.40 (0.55)
%  & 10.92 (0.79) 
%  & \bf 9.47 (0.82)  
%  & 10.37 (0.81)
%  & 10.71 (0.79)
%  & \bf 9.47 (0.82) 
% \\ \bottomrule
% \end{tabular}
% }
% \vspace{-5pt}
% \caption{Ablation studies on different components, modalities and scoring tokens. The value outside the brackets is MSE while inside is Spearman correlation.
% % For component part, \textbf{B}: Baseline; \textbf{TA}: Token Aggregation; \textbf{MRU}: Memory Recurrent Unit; \textbf{Bi-D}: Bi-direction. Figure~\ref{fig:abl_structure} shows the detailed comparison.
% }
% \vspace{-10pt}
% %. For the number of Layers experiments are conducted on 1, 2 and 3 Mixer Layers. For dropout rate, 0\%, 10\%, 20\% and 30\% are analyzed here.}
% \label{fig:abl} \end{table*}

% \subsubsection{Modality.}
\noindent\textbf{Modality. }
Here we analyze the importance of using multimodal information in figure skating task. We have run experiments on our proposed model with only audio and only visual features. 
Results in Table~\ref{fig:abl} show that Skating Mixer with only audio features generates the worst result. %This follows our intuition that music plays an auxiliary part in figure skating. 
This follows the commonsense that music plays an auxiliary part in figure skating and the visual technique moves always play the key role for scoring. 
% Using both audio and video clues in Skating Mixer performs better than using only visual features. 
% Introducing both audio and video clues in figure skating scoring performs better than using only visual features, especially in \textbf{\emph{PCS}}.
Introducing both audio and video clues in figure skating scoring performs better than using only visual features, which further demonstrates that audio-visual learning is really important in this field.
% It is surprised to see that the audio feature could also slightly improve the performance on \textbf{\emph{TES}} which only measures the difficulty and completion of the action without considering the musical elements according to the scoring rules. This implies that music might also slightly affect referees' decision when giving \textbf{\emph{TES}}.
% Similar to the result on Fis-V, model using only acoustic features provide little information and obtain the worst result, because the technique moves (in video) always play the key role for scoring. However, the advantage that using multimodality in our model is very obvious, which further demonstrates that audio-visual learning is really important in this field.
%The music may provide additional clues to identify the category of figure skating and lead the model to use different scoring schemes for different videos.
%\mc{We believe that this is because music may provide additional clues to identify the category of figure skating, and help the model to judge the player's expression to them. }

\noindent\textbf{Scoring token. }
% \subsubsection{[CLS] \& [MEM] token.}
In this section, we are going to discuss the effectiveness of \texttt{[CLS]} and \texttt{[MEM]} token in our proposed architecture. In our model, both $\texttt{[CLS]}$ and $\texttt{[MEM]}$ token output are used for final scoring. We first generate scores with only the output from CLS Mixer, which means only \texttt{[CLS]} token outputs are used for scoring. Then we utilize only the \texttt{[MEM]} output from the last clip for scoring. The result show that using both $\texttt{[CLS]}$ and $\texttt{[MEM]}$ token generates the best result. 
% The intuition behind this setting is that the output of \texttt{[CLS]} token contains the local information while the \texttt{[MEM]} includes the global information of the whole video.
This is because $\texttt{[MEM]}$ token passes across the whole video and contains global information while $\texttt{[CLS]}$ token contains local information of each clip. 
Combining these two types of features could improve the performance.
% First, we remove the \texttt{[CLS]} token and only use the output of \texttt{[MEM]} in the last clip to predict the score. The output of \texttt{[MEM]} passes through the scoring head, which is an MLP layer, and generates the score. 
% The intuition behind this setting is that the output of \texttt{[CLS]} token contains the local information while the \texttt{[MEM]} includes the global information of the whole video. It is expected to improve the performance by combining these two kinds of information.
% % Here we analyze the result on \textbf{\textit{TES}} and \textbf{\textit{PCS}} for both datasets.
% However, from the results in Table~\ref{tab:abl} we can find that using two tokens in the scoring head could obtain better result of \textbf{\textit{TES}} on the FS1000 dataset but it does not perform well on the other metrics. 
% The reason is that during the token mixing process, \texttt{[CLS]} and \texttt{[MEM]} are already interacted with each other and do not need further fusion inside the scoring head.
% It also shows that utilizing only \texttt{[MEM]} cannot achieve
% obvious improvement as it leaves out the local information. Therefore, we directly use the output of \texttt{[CLS]} token in the scoring head in other experiments. %\mc{Since the motivation of us is to desgin a general multimodal MLP architecture without any complex modules, so we finally use \texttt{[CLS]}. }
% \vspace{-20pt}

\noindent\textbf{Backbones.}
% \begin{table}[h!]
% \scriptsize
% \centering
% % \setlength\tabcolsep{1.82pt}
% % \renewcommand\arraystretch{1.0}
% \scalebox{0.9}{
% \begin{tabular}{l|c|cccc}
% \toprule
% \rowcolor{blue!10}
%   \multicolumn{1}{c|}{\textbf{Dataset}} &
%   \multicolumn{1}{c|}{\textbf{Backbone}} &
%   \multicolumn{1}{c}{\textbf{\textit{TES}}} &
%   \multicolumn{1}{c}{\textbf{\textit{PCS}}} &
%   \multicolumn{1}{c}{\textbf{\# Params}} &
%   \multicolumn{1}{c}{\textbf{MACs}}\\ \hline
% % \rowcolor{blue!10}
% % \multicolumn{2}{l|}{}    & \textbf{C3D[]} & \textbf{TimeSformer[]} & \textbf{C3D[]} & \textbf{TimeSformer[]}  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fis-V\\ \end{tabular}} &
%   Transformer & 25.60 (0.51)
%   & 13.18 (0.68)
%   & 20.48M
%   & 35.55G
%     \\
%  & MLP-Mixer & \bf 19.57 (0.68) & \bf 7.96 (0.82) & \bf 14.25M & \bf 24.95G    \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}FS1000\\ (Ours)\end{tabular}} &
%   Transformer & 120.24 (0.81)
%      & 13.40 (0.76)
%      & 20.48M
%      & 48.92G
%   \\
%  & MLP-Mixer & \bf 81.24 (0.88) & \bf 9.47 (0.82) & \bf 14.25M  & \bf 34.36G 
% \\ \bottomrule
% \end{tabular}
% }
% % \vspace{5pt}
% \caption{Comparison of Transformer and MLP-Mixer as backbone in our Skating Mixer.}
% % \vspace{-20pt}
% %. For the number of Layers experiments are conducted on 1, 2 and 3 Mixer Layers. For dropout rate, 0\%, 10\%, 20\% and 30\% are analyzed here.}
% \label{tab:backbone} \end{table}
% The input and output of CNN have different shapes and thus cannot find the position of mem token and cls token output.
In this part, we show the difference between MLP-Mixer and Transformer.
Transformer has been widely adopted in the multimodal area, but as mentioned in~\cite{tolstikhin2021mlp}, the computation complexity of Transformer is $\mathcal{O}(n^2)$ while for MLP-Mixer it is $\mathcal{O}(n)$, where $n$ is the number of input tokens.
Also, \cite{Liu2021EfficientTO} mentions that Transformer usually requires large amount of data for training.
% In fact, MLP-based architecture is found to be superior in our task.
%Also, in our case, Transformer does not necessarily reduce the number of parameters since calculating multi-head attention also needs multiple MLPs. 
% Besides, experiments also show that MLP-based architecture is found to be superior in our task (Shown in Table~\ref{tab:backbone}).
% Due to the recurrent strategy, the number of input tokens is small so token-mixing MLP (L311) . 
We conduct experiments by replacing the MLP-Mixer with the same number of Transformer blocks. 
The results in Table~\ref{tab:backbone} demonstrate that in our task with a relatively small dataset (compared to Imagenet~\cite{imagenet_cvpr09}), MLP-Mixer yields better performance than Transformer with less computation resource.
% Moreover, MLP-Mixer is more computation efficient than Transformer in this case. 
% Additionally, we can see that   
% MLP-Mixer with fewer parameters yields better results. 


% \begin{table}[h]
% \scriptsize
% \centering
% % \setlength\tabcolsep{1.82pt}
% % \renewcommand\arraystretch{1.0}
% \scalebox{0.9}{
% \begin{tabular}{l|c|cccc}
% \toprule
% \rowcolor{blue!10}
%   \multicolumn{1}{c|}{\textbf{Dataset}} &
%   \multicolumn{1}{c|}{\textbf{Backbone}} &
%   \multicolumn{1}{c}{\textbf{\textit{TES}}} &
%   \multicolumn{1}{c}{\textbf{\textit{PCS}}} &
%   \multicolumn{1}{c}{\textbf{\# Params}} &
%   \multicolumn{1}{c}{\textbf{MACs}}\\ \hline
% % \rowcolor{blue!10}
% % \multicolumn{2}{l|}{}    & \textbf{C3D[]} & \textbf{TimeSformer[]} & \textbf{C3D[]} & \textbf{TimeSformer[]}  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fis-V\\ \end{tabular}} &
%   Transformer & 25.60 (0.51)
%   & 13.18 (0.68)
%   & 
%   & 
%     \\
%  & MLP-Mixer & 19.57 (0.68) & 7.96 (0.82)  &   &      \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}FS1000\\ (Ours)\end{tabular}} &
%   Transformer & 113.24 (0.81)
%      & 13.40 (0.76)
%      & 
%      &
%   \\
%  & MLP-Mixer & 81.24 (0.88) & 9.47 (0.82) &   &  
% \\ \bottomrule
% \end{tabular}
% }
% % \vspace{5pt}
% \caption{Comparison of different backbones.}
% \vspace{-20pt}
% %. For the number of Layers experiments are conducted on 1, 2 and 3 Mixer Layers. For dropout rate, 0\%, 10\%, 20\% and 30\% are analyzed here.}
% \label{tab:backbone} \end{table}

% \noindent\textbf{Feature Extractor.}
% % \textbf{Feature Extractor.}
% %In addition to the model pre-trained on Kinetics~\cite{kay2017kinetics}, 
% % TimeSformer provides pre-trained weights on Kinetics~\cite{kay2017kinetics} and HowTo100M~\cite{miech2019howto100m}.
% % HowTo100M dataset contains much longer videos than Kinetics.  
% % Though this factor is not at the core of our design, we are interested to see whether it plays an important role.
% % %We can see that although HowTo100M pre-trained model achieves better MSE loss in FS1000, for most of the time, using Kinetics~\cite{kay2017kinetics} pre-trained model generates better results. So we adopt this setting in other experiments.
% % As shown in Figure~\ref{fig: fe_abl}: for most of the time, using Kinetics~\cite{kay2017kinetics}-based model performs better. So we adopt this setting.
% \begin{figure}[t!]
% \centering
% % \begin{minipage}[t]{0.48\textwidth}
% % \centering
% % \includegraphics[width=0.48\linewidth]{image/TES.pdf}\label{fig:loss}
% % \includegraphics[width=0.48\linewidth]{image/PCS5.pdf}\label{fig:extractor}
% % \caption{Loss plots of the early 30 epochs when training on Fis-V. %Solid line refers to our proposed method and dotted lines are LSTM-based methods~\cite{xu2019learning}. Training our method converges much faster than other models.
% % }
% % \label{fig: process}
% % \end{minipage}
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \includegraphics[width=0.95\linewidth]{image/fe_ZGMC.pdf}
% \caption{Results when applying different feature extractors on both datasets.}
% \label{fig: fe_abl}
% \end{minipage}
% \vspace{-10pt}
% \end{figure}
% Besides using AST and Timesformer as feature extractor, we also adopt Vggish~\cite{vggish} and C3D~\cite{c3d} to extract features and here we demonstrate the result in Figure~\ref{fig: fe_abl}. Experiments have shown that different feature extraction affects final performance, but our Skating-Mixer can perform admirably in all cases.

% \noindent\textbf{Number of Mixer Layer.}
% \textbf{Number of Mixer Layer.}
% % On Fis-V dataset, since the dataset is relatively small and just has a single category of figure skating, we just apply one Mixer layer in our Skating Mixer. However, FS1000 dataset contains more complicated and diverse information, totally eight types of competitions, so we add one more Mixer layer, namely two Mixer layers as our setting in the experiments on FS1000 dataset, which can further effectively improve the performance.
% %We also analyze the result when using different number of MLP-Mixer layers in our proposed structure. 
% We also conduct the experiments using different numbers of MLP-Mixer layers in our proposed structure.
% Insufficient Mixer layers would lead the model to miss some important information while too many Mixer Layers will cause over-fitting problems on the task-specific dataset.
% As the result shown in Table~\ref{fig:abl}, on both datasets, two MLP-Mixer layers are the best setting in our model. % It can also be observed that when using three Mixer layers, it causes serious over-fitting problem and the performance becomes much worse for most of the time.
% We argue that using three Mixer layers causes serious over-fitting problems and the performance becomes much worse.
% As the result shown in Table~\ref{}, on Fis-V dataset, two MLP-Mixer layers is enough since Fis-V is a relatively small dataset and contains only  a single category of figure skating. However, FS1000 dataset contains more complicated and diverse information, totally eight types of competitions, so two Mixer layers can further effectively improve the performance.

% \noindent\textbf{Setting of Dropout Rate.}
% \textbf{Setting of Dropout Rate.}
% %In our experiment, we observe that with a small dataset, our model is getting over-fitted easily. 
% %One possible solution is to introduce the dropout mechanism into our model. 
% Since the figure skating videos are really long, we worry about the over-fitting problem at first.  So dropout layers have been introduced before and after both channel-mixing MLP and token-mixing MLP.
% %
% %We set the dropout rate to be $0\%$,  $10\%$, $20\%$ and $30\%$ and test the model on both Fis-V and FS1000 datasets. 
% We set the dropout rate to be $0\%$,  $10\%$, $20\%$ and $30\%$.
% Results are shown in Table~\ref{fig:abl}: %On FS1000 dataset\mc{:} introducing the dropout mechanism \mc{decreases} the MSE for \mc{\textbf{\emph{TES}}}. \mc{But} \mc{\textbf{\emph{TES}}} gets the best result when the dropout rate is 0.1. However, the dropout strategy will increase the MSE for \mc{\textbf{\emph{PCS}}}. On Fis-V dataset we find that the model without dropout layers performs the best on both \mc{\textbf{\emph{TES}}} and \mc{\textbf{\emph{PCS}}}. In conclusion dropout layers do not alleviate the over-fitting problem and even deteriorate the performance in most cases.
% different from other tasks~\cite{He_2016_CVPR, vaswani2017attention, nakano2020estimating}, using a higher dropout rate cannot achieve obvious improvements in this scenarios.
% This may demonstrate that keeping the feature continuous and comprehensive is important for scoring figure skating since every move is important. 


==> LaTeX/Section/05_Experiment/dataset.tex <==
% \subsection{Result on different datasets}
%First, we compare our Skating-Mixer with MS-LSTM on both Fis-V~\cite{xu2019learning} and FS1000 dataset. 
% In the original paper, it reports the best result it got. 

% C3D features are used in the LSTM-based structure as in ~\cite{xu2019learning}. We also run experiments on S-LSTM and M-LSTM mentioned before.
%Our model is compared with previous figure skating scoring methods~\cite{parmar2017learning,parmar2019action,xu2019learning} and a supervised audio-visual Transformer-based method~\cite{lee2020parameter}.


In this section, we show the experiment results on Fis-V dataset and FS1000 of different methods.
Fis-V dataset~\cite{xu2019learning} contains 400 ladies short program videos for training and 100 videos for validation. 
%The raw videos are released in their GitHub repository.
% The raw videos from Fis-V dataset contain both 30 fps and 25 fps format, so we convert 30 fps video to 25 fps.
Our proposed FS1000 dataset contains a training set of 1000 videos and a validation set of 247 videos.
% For a fair and accurate comparison, we run 3 repeated experiments using different random seeds and record the mean of metrics for different methods~\cite{xu2019learning,parmar2017learning,parmar2019action,lee2020parameter}. 
AST~\cite{gong2021ast} and TimeSformer~\cite{bertasius2021spacetime} are used as our feature extractor.
The Mean Square Error (MSE) and Spearman Correlation are used as our evaluation metrics. 
We compare our method with several related methods~\cite{xu2019learning,parmar2017learning,parmar2019action,lee2020parameter}.
M-Bert~\cite{lee2020parameter} uses both audio and visual features while others only consider visual features.
It should be noted that we find around 40 out of 500 videos in Fis-V~\cite{xu2019learning} dataset contains redundant information (such as the interview and replay), so we cut the videos and re-extract the features. 
% Additionally, MS-LSTM~\cite{xu2019learning} randomly cropped 300 frames of input features for training and testing. In this case, these methods could have bias (as they only see a random part of the competition) and produce inaccurate results. So in our experiment, we modify the models and use all the features as input.
% S-LSTM contains only self-attention part in MS-LSTM while M-LSTM contains only multi-scale part.
%We also included S-LSTM and M-LSTM, which contains part of the structure of MS-LSTM in ~\cite{xu2019learning} as they perform better in some of the experiments.
%For the Transformer-based model, we also analyzed the early, mid and late fusion strategy which has been discussed widely in audio-visual learning~\cite{nagrani2021attention}.
% We also conduct experiments on our model with only acoustic modality or visual modality. We record  the comprehensive results in Table~\ref{tab: fs1000-reb}.

% \noindent{\textbf{Fis-V.}}
% \textbf{Fis-V.}
\vspace{-2pt}
\input{Section/05_Experiment/exp_fisv}

% \noindent{\textbf{FS1000.}}
% \textbf{FS1000.}
\vspace{-2pt}
\input{Section/05_Experiment/exp_fs1000}




% \noindent\textbf{Summary. } 
% \textbf{Summary. } 
% It can be found that learning to score figure skating videos requires the model to learn both long-term dependency and multimodality learning. Transformer is a popular form for modal interaction, but it is hard to handle such long videos; LSTM-based method performs better in some datasets, but it fails to introduce multimodality and generalize across different categories. Our model is capable of dealing with these two aspects at the same time and performs better than CNN, LSTM and Transformer-based models. We believe the new neural network could be used for more than scoring figure skating but also a pioneer work utilizing MLP-based model for multimodal learning in long videos.

==> LaTeX/Section/05_Experiment/exp_fisv.tex <==
\subsection{Results on Fis-V}
From Table~\ref{tab: fs1000-reb}, it can be observed that our proposed Skating-Mixer outperforms CNN-based~\cite{parmar2017learning, parmar2019action}, LSTM-based~\cite{xu2019learning,parmar2017learning} and Transformer-based~\cite{lee2020parameter} models. Although the Transformer model performs better than MLP-Mixer on general tasks like image classification~\cite{tolstikhin2021mlp}, it does not have an obvious advantage in this specific task. C3D-LSTM~\cite{parmar2017learning} has the worst results since the model is too simple to learn such complex data. 3D CNN-based method, MSCADC~\cite{parmar2019action} is also struggled to understand such long videos. 
%MS-LSTM and our proposed Skating Mixer performs better than Transformer model, indicating that the memory recurrent unit plays an essential role in long videos learning. 
MS-LSTM~\cite{xu2019learning} and our proposed Skating Mixer performs better than Transformer model, indicating that: a strong memory mechanism plays an essential role in long videos learning; besides, the attention mechanism is less effective to capture extremely long-term dependencies across clips over several minutes. 
Additionally, by comparing our model and M-Bert~\cite{lee2020parameter}, it could be found that our model could better learn multimodal features from long videos.
% Moreover, our model with only video feature can still achieves better results than MS-LSTM~\cite{xu2019learning}, proving that our structure
% learns better in long video information.
%can better obtain long-video information.
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=0.25\linewidth]{image/TES.pdf}
% %   \hspace{1in}
%   \includegraphics[width=0.25\linewidth]{image/PCS5.pdf}
%   \caption{The loss plots of the first 30 epochs when training on Fis-V. Solid line refers to our proposed method and dotted lines are LSTM-based methods~\cite{xu2019learning}. Training our method converges much faster than other models.}
%   \label{fig: process}
%   \vspace{-15pt}
% \end{figure}

% Additionally, Skating Mixer with only audio features generates the worst result. %This follows our intuition that music plays an auxiliary part in figure skating. 
% This follows the commonsense that music plays an auxiliary part in figure skating. 
% % Using both audio and video clues in Skating Mixer performs better than using only visual features. 
% Introducing both audio and video clues in figure skating scoring performs better than using only visual features, especially in \textbf{\emph{PCS}}. It is surprised to see that the audio feature could also slightly improve the performance on \textbf{\emph{TES}} which only measures the difficulty and completion of the action without considering the musical elements according to the scoring rules. This implies that music might also slightly affect referees' decision when giving \textbf{\emph{TES}}.
% \begin{figure}
%   \centering
%   \includegraphics[width=0.49\linewidth]{latex/image/TES.pdf}
% %   \hspace{1in}
%   \includegraphics[width=0.49\linewidth]{latex/image/PCS5.pdf}
%   \caption{The loss plots of the first 30 epochs when training on Fis-V. Solid line refers to our proposed method and dotted lines are LSTM-based methods. Our method converges much faster than previous ones.}
%   \label{fig: process}
%   \vspace{-10pt}
% \end{figure}

==> LaTeX/Section/05_Experiment/exp_fs1000.tex <==
\subsection{Results on FS1000}
Scoring on the FS1000 dataset is much more challenging since Fis-V~\cite{xu2019learning} dataset only contains ladies short program videos while FS1000 dataset consists of different types of figure skating videos, which highly tests the robustness of model. 
%\mc{And, different categories of figure skating have different technical moves with different scores.}
%and the scoring standards for different types are slightly different, 
%especially t
%\mc{T}he scoring of\textbf{\emph{TES}} 
%since different categories of figure skating have different technical moves with different scores.
%However, the quality and completion of each actions and the matching degree between music and video are something in common across different categories.
% For example, ice skating values more on how music matches skating movement compared to pairs skating and pairs program should also considers the synchronization of two athletes compared to individual skating.
% We train our model on the FS1000 dataset to predict figure skating scores of different competitions, and the models with a single modality are also trained and evaluated.
%\textcolor{red}{As mentioned before, the factor is a pre-defined value to adjust the weight of \mc{\textbf{\emph{PCS}}} in a certain category of figure skating, so the \mc{\textbf{\emph{PCS}}} scores are normalized by a factor into the same scale.} Five sub-scores are also included in our experiment.
% The performance on FS1000 dataset is also evaluated by MSE.
%The experiment results show that our proposed Skating Mixer achieves better results than other models by a large margin.
As shown in Table~\ref{tab: fs1000-reb}, CNN-based~\cite{parmar2017learning,parmar2019action} and Transformer-based~\cite{lee2020parameter} models still cannot capture long-term dependencies across extremely long videos. 
LSTM-based~\cite{xu2019learning} models achieves better results but fails to further improve the results with only visual features.
% MS-LSTM~\cite{xu2019learning}, which achieves closer performance to our model on Fis-V dataset, obviously fails to extend to multi-category FS1000 dataset, especially in \textbf{\emph{TES}}. We conclude that it is because MS-LSTM~\cite{xu2019learning} cannot well uncover the underlying relationships for different categories. 
Our proposed model could handle multimodal information in long figure skating videos and shows great flexibility to fit different types of competitions and obtain the best result among all the models.
% Similar to the result on Fis-V, model using only acoustic features provide little information and obtain the worst result, because the technique moves (in video) always play the key role for scoring. However, the advantage that using multimodality in our model is very obvious, which further demonstrates that audio-visual learning is really important in this field.
%The music may provide additional clues to identify the category of figure skating and lead the model to use different scoring schemes for different videos.
%\mc{We believe that this is because music may provide additional clues to identify the category of figure skating, and help the model to judge the player's expression to them. }
Another interesting observation is that performance score \textbf{\emph{PE}} is harder to learn than other four sub-scores for all the models, indicating that future work could focus on improving the learning of performance score for a better overall result.
%the scoring standard for performance is obscure for this score. 

==> LaTeX/Section/05_Experiment/experiment_setting.tex <==
% \subsection{Implementation Details}

% % \textbf{Dataset.}
% \subsubsection{Dataset.}
% In this section, we first test our model on Fis-V dataset~\cite{xu2019learning} which contains 400 ladies short program videos for training and 100 videos for validation. 
% %The raw videos are released in their GitHub repository.
% % The raw videos from Fis-V dataset contain both 30 fps and 25 fps format, so we convert 30 fps video to 25 fps.
% Then, we evaluate our model on our proposed FS1000 dataset. %In the FS1000 dataset, we split 652 videos as the training set and 160 videos as the validation set. 
% We used 1247 videos from the FS1000 dataset and divided into a training set of 1000 videos and a validation set of 247 videos.

% % \noindent{\textbf{Feature Extraction Setting.}}
% \textbf{Feature Extraction Setting.}
% In our experiment, all the video data have 25 frames per second. Each video is separated into a 5-second clip and adjacent clips have 3 seconds overlapping time duration. The overlapping setting tends to avoid inconsistency caused by splitting. 
% For feature extraction, we use the Audio Spectrogram Transformer~\cite{gong2021ast} pre-trained on full AudioSet~\cite{audioset} to extract acoustic features. For the visual feature, TimeSformer~\cite{bertasius2021spacetime} pre-trained on Kinetics-600 dataset~\cite{kay2017kinetics} is implemented. 
% In the original paper, the number of input frames of TimeSformer is 8, so we also adopt the same setting here. 
% %
% To round up that 125 cannot be divided by 8, we take 120 frames from 125 frames for each clip.
% So each clip is separated into 15 non-overlapping 8-frame segments and each segment is input into the model. 
% In other words, there will be 15 tokens used as the visual representation for each clip. We do not fine-tune both Transformers on Fis-V and our dataset because of tremendous computational cost and memory usage. Figure skating videos contain up to 6000 frames and it will require $\sim$200G memory and more than 2 minutes for a single video to pass forward and backward the model. Thus they are not included in our training graph.

% % \noindent{\textbf{Model Setting.}}
% \textbf{Model Setting.}
% In our experiment, %we use one MLP-Mixer layer in the recurrent structure on Fis-V dataset and two layers on FS1000 dataset.
% we use two MLP-Mixer layer in the recurrent structure.
% %The batch size is 16 and the optimizer is Adam with learning rate 0.0001. 
% Adam optimizer with learning rate $1e-4$ is deployed. The scoring head $\text{ScoreHead}$($\cdot$) is a simple linear layer. For completed learning, the whole framework is trained with 500 epochs on a single NVIDIA V100. 

% \textbf{Metrics.}
% In our experiment, we use Mean Square Error (MSE) and Spearman Correlation, which is commonly used in figure scoring task~\cite{xu2019learning, parmar2017learning}. Mean Square Error is a metric used to measure the value difference between the true score and the predicted score. Spearman correlation is a non-parametric metric to show the monotonicity of the relationship between two variables. In our case, we use this metric to calculate if the predicted results and the true results are similar to each other in ranking or not. Suppose the predicted score is $P$ and the true score is $T$. The number of samples is $N$. The equation of MSE could be written as:
% \begin{equation*}
% MSE=\frac{1}{N} ||P - T||^2_2
% \end{equation*}
% Smaller MSE indicates more accurate prediction.
% To calculate the Spearman correlation, we first convert raw scores to rank $\mathrm{R}(P)$ and $\mathrm{R}(T)$.
% The coefficient $r_{s}$ is computed as follow:
% \begin{equation*}
% r_{s}=\frac{\operatorname{cov}(\mathrm{R}(P), \mathrm{R}(T))}{\sigma_{\mathrm{R}(P)} \sigma_{\mathrm{R}(T)}}
% \end{equation*}
% A higher coefficient value means a better rank correlation between the true and predicted scores. 
% The result is demonstrated in Table~\ref{tab: spearman}. We can still see that our method outperforms other methods and the multimodal model generates better results compared to the model with a single modality.

==> LaTeX/Section/05_Experiment/manuscript.tex <==
\input{Section/05_Experiment/experiment_setting}


\begin{table*}[!t]
%\normalem
%   \vspace{-6pt}
	\renewcommand\tabcolsep{5.4pt}
	\centering
	\small
	\scalebox{0.9}{
        \begin{tabular}{c|c|ccccccc|ccccccc}
        \toprule
        \rowcolor{blue!10}
         \multicolumn{1}{c|}{\textbf{Datasets}}&
         \multicolumn{1}{c|}{\textbf{Methods}} & &       &   \multicolumn{3}{c}{\textbf{\emph{Mean Square Error}($\downarrow$)}}   &  & &  & \multicolumn{5}{c}{\textbf{\emph{Spearman Correlation}($\uparrow$)}} &  \\ \cline{3-16}
         \rowcolor{blue!10}
          & 
          & \multicolumn{1}{c}{\textbf{\emph{TES}}}   &  \multicolumn{1}{c}{\textbf{\emph{PCS}}}     & \multicolumn{1}{c}{\textbf{\emph{SS}}}   &  \multicolumn{1}{c}{\textbf{\emph{TR}}}& \multicolumn{1}{c}{\textbf{\emph{PE}}}   &  \multicolumn{1}{c}{\textbf{\emph{CO}}}& \multicolumn{1}{c|}{\textbf{\emph{IN}}} & \multicolumn{1}{c}{\textbf{\emph{TES}}}   &  \multicolumn{1}{c}{\textbf{\emph{PCS}}}     & \multicolumn{1}{c}{\textbf{\emph{SS}}}   &  \multicolumn{1}{c}{\textbf{\emph{TR}}}& \multicolumn{1}{c}{\textbf{\emph{PE}}}   &  \multicolumn{1}{c}{\textbf{\emph{CO}}}& \multicolumn{1}{c}{\textbf{\emph{IN}}}  \\ \hline
       & C3D-LSTM & 39.25 & 21.97 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & 0.29 & 0.51 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$\\
      & MSCADC& 25.93 & 11.94 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & 0.50 & 0.61 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$\\ \cline{2-16}
      & M-LSTM & 25.70 & 12.48 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$& 0.53 & 0.68 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$\\
      & S-LSTM & 22.31 & 10.21 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$& 0.57 & 0.74 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$\\
      Fis-V& MS-LSTM & 22.64 & 9.84 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$& 0.59 & 0.73 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$\\ \cline{2-16}
      & M-BERT (Early)  & 28.04  &  13.31 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$& 0.54 & 0.69 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$  \\ 
      & M-BERT (Mid)  & 33.32 & 17.79 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & 0.54 & 0.71 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$        \\
      & M-BERT (Late)  & 27.73 & 12.38 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & 0.53 & 0.72 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$      \\  \cline{2-16}
    %   & Ours (A)  &  &  & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$  &  &  & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$  \\ 
    %   & Ours (V)  &  20.45 & 9.03 &$\dagger$  &$\dagger$  &$\dagger$  &$\dagger$  & $\dagger$  &  &  & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$         \\ 
      & Ours  &\bf 19.57 & \bf 7.96 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & \bf 0.68 & \bf 0.82 & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$ & $\dagger$\\ \midrule
      & C3D-LSTM & 308.30 & 25.85 & 0.92 & 0.99 & 1.21 & 0.97 & 1.01 & 0.78 & 0.53 & 0.50 & 0.52 & 0.52 & 0.57 & 0.47\\
      & MSCADC & 148.02 & 15.47 & 0.51 & 0.57 & 0.78 & 0.55 & 0.60 & 0.77 & 0.70 & 0.69 & 0.69 & 0.71 & 0.68 & 0.71\\
        \cline{2-16}
      & M-LSTM  & 104.62 & 15.57 & 0.49 & 0.72 & 0.89 & 0.46 & 0.56 & 0.84 & 0.69 & 0.74 & 0.59 & 0.64 & 0.78 & 0.71  \\  
      & S-LSTM  & 83.79 & 10.90 & 0.40 & 0.43 & 0.70 & 0.40 & 0.44 & 0.87 & 0.79 & 0.79 & 0.80 & 0.78 & 0.80 &    0.80   \\  
      FS1000 (Ours) & MS-LSTM  & 94.55 & 11.03 & 0.45 & 0.49 & 0.76 & 0.43 & 0.47 & 0.86 & 0.80 & 0.77 & 0.78 & 0.76 & 0.79 & 0.78       \\  \cline{2-16}
      & M-BERT (Early)  & 139.09 & 14.49 & 0.44 & 0.44 & 0.71 & 0.47 & 0.50 & 0.78 & 0.77 & 0.80 & 0.80 & 0.76 & 0.79 & 0.79        \\ 
      & M-BERT (Mid)  & 170.57 & 21.28 & 0.57 & 0.54 & 0.69 & 0.56 & 0.56 & 0.77 & 0.75 & 0.79 & 0.79 & 0.80 & 0.79 & 0.80         \\ 
      & M-BERT (Late)  & 131.28 & 15.28 & 0.44 & 0.43 & 0.67 & 0.47 & 0.55 & 0.79 & 0.75 & 0.80 & 0.81 & 0.80 & 0.80  & 0.76         \\ \cline{2-16}
    %   & Ours (A) &  &  &  &  &  &  &  &  &  &  &  &  &  &           \\ 
    %   & Ours (V) & 68.16 & 11.56 & 0.42 & 0.48 & 0.84 & 0.49 & 0.55      & 0.85 & 0.82 & 0.80 & 0.80 & 0.78 & 0.78 & 0.74     \\ 
      & Ours   & \bf 81.24  & \bf 9.47 & \bf 0.35 & \bf 0.35 & \bf 0.62 & \bf 0.37 &   \bf 0.39 & \bf 0.88 & \bf 0.82 & \bf 0.80 & \bf 0.81 & \bf 0.80 & \bf 0.81 & \bf 0.81  \\ 
      \bottomrule
        \end{tabular}}
\vspace{-5pt}
\caption{Experiment Results on Fis-V~\cite{xu2019learning} and ours FS1000. \textbf{CNN-based}: \cite{parmar2017learning, parmar2019action}, \textbf{LSTM-based}:~\cite{xu2019learning,parmar2017learning}, \textbf{Transformer-based}:~\cite{lee2020parameter}, \textbf{MLP-based}: Ours. 
MSE and Spearman Correlation are used for evaluation. For MSE, the lower the better; for Spearman Correlation, the higher the better.
% The scores are computed by MSE. 
% A: only audio, V: only video, A+V: Audio+Video.
$\dagger$ denotes the dataset does not include the GT.}
\vspace{-15pt}
\label{tab: fs1000-reb}
\end{table*}


% \input{Sections/Experiment/exp_fisv}

% \input{Sections/Experiment/exp_fs1000}
\input{Section/05_Experiment/dataset}

% \input{Sections/Experiment/one_model}
\vspace{-3pt}
\input{Section/05_Experiment/ablation}

\input{LaTeX/Section/05_Experiment/visualization}

\input{Section/05_Experiment/ranking}

==> LaTeX/Section/05_Experiment/ranking.tex <==
\vspace{-4pt}
\subsection{Performances on Beijing 2022 Olympic Games}
To verify the robustness and effectiveness of the figure skating model, %it is necessary to apply our trained model on competitions that is not included in the dataset to see its actual effect. 
we apply our trained model on competitions that are not included in the training data to see its actual effect. 
Therefore, we take the figure skating videos from the Beijing 2022 Winter Olympic Games and make analysis on the rankings of athletes. In practice, predicting correct ranking is more meaningful than predicting the exact scores because the evaluation scales are inconsistent on different competitions. Here we use our model to predict the \textbf{\emph{PCS}} for samples. Figure~\ref{fig:rank} demonstrates the results of Ladies Short and Pair Free program. It shows that although the score may not be accurate, the top-5 ranking does not change too much compared to real ranking. This is because top-tier athletes share similar technique moves and maintain high-quality performances. 
Such results could satisfy the practical need for auxiliary judgment.
This demonstrates that our model could actually learn some of the scoring standards and identify better performance from a group of athletes. 
%since referees could hardly agree on the same score most of the time.
%\subsection{Testing result on 2022 Olympics}
% \begin{figure}[h]
% \begin{center}
% % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \includegraphics[width=1.0\linewidth]{image/rank_ZGMC.pdf}
% \end{center}
% \vspace*{-10pt}
%     \caption{Predicted TOP-5 Ranking for Ladies Short in Beijing 2022 Winter Olympic Games. $P$ stands for predicted and $T$ stands for truth. The last row is the ranking difference compared to the real ranking.}
% \label{fig:LS ranking}
% \vspace{-15pt}
% \end{figure}

% \begin{figure}[h]
% \begin{center}
% % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \includegraphics[width=\linewidth]{image/ls_2022_lstm.pdf}
% \end{center}
% \vspace*{-10pt}
%     \caption{Predicted TOP-5 Ranking for Ladies Short Program in Beijing 2022 Winter Olympic Games with MS-LSTM~\cite{xu2019learning}. The model generates much worse results compared to our model.}
% \label{fig:LS lstm}
% \vspace{-15pt}
% \end{figure}
%since the regulation of \mc{\textbf{\emph{TES}}} changes from season to season and our training dataset are base on competitions before 2019.
% Figure~\ref{fig:LS ranking} shows the result of our Skating Mixer and MS\_LSTM~\cite{xu2019learning} on Ladies Short program. Both of the models are trained on Fis-V~\cite{xu2019learning} dataset and directly predict the scores. 
% The ranking is assigned according to the predicted scores. We compare the result with the real ranking. 
% From the result, we can see that our model performs much better than MS\_LSTM.
%The Skating Mixer trained on Fis-V~\cite{xu2019learning} dataset is used to predict the score in Ladies Short Program. The top 5 athletes are presented according to our prediction.
% 
%However, for top athletes who get much higher score than others, the score difference would not affect the rankings much; for those athletes who have similar scores, the model may have different results. %More accurate methods are still needed.
% \begin{figure}[h]
% \begin{center}
% % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \includegraphics[width=1.0\linewidth]{LaTeX/image/visualization1.pdf}
% \end{center}
% \vspace*{-10pt}
%     \caption{Score difference when sequentially adding clips. The score is low when the action is failed (blue box); the score is relatively high when finishing a complex move (yellow box) or skate fluently with the music (green box).}
% \label{fig:visualization}
% \vspace{-10pt}
% \end{figure}

\begin{figure}[t]
\centering
\subfigure[Predicted results on Ladies Short Program]{
\includegraphics[width=\linewidth]{LaTeX/image/score_rank_LS.pdf}
%\caption{fig1}
}
\quad
\subfigure[Predicted results on Pairs Free Program]{
\includegraphics[width=\linewidth]{LaTeX/image/score_rank_PF.pdf}
}
\vspace{-5pt}
\caption{Predicted TOP-5 Ranking in Beijing 2022 Winter Olympic Games. $P$ stands for predicted score and $T$ stands for true score. The last row is the ranking difference compared to the real ranking.}
\label{fig:rank}
\vspace{-15pt}
\end{figure}

% \begin{figure}[h]
% \centering
% \subfigure[Predicted results with Skating Mixer trained on Fis-V dataset~\cite{xu2019learning}.]{
% \includegraphics[width=\linewidth]{image/pf_2022_fisv.pdf}
% %\caption{fig1}
% }
% \quad
% \subfigure[Predicted results with Skating Mixer trained on FS1000 dataset.]{
% \includegraphics[width=\linewidth]{image/pf_2022.pdf}
% }
% \caption{Predicted TOP-5 Ranking for Pairs Free Skating in Beijing 2022 Winter Olympic Games.}
% \label{fig:PF ranking}
% \end{figure}


% Moreover, we applied MS-LSTM~\cite{xu2019learning}, which has a closer performance to our model, to the videos in Winter Olympic Games. The result is demonstrated in Figure~\ref{fig:LS lstm}. We can see that the predicted ranking result is much worse than that when using our proposed structure. This obviously shows that our proposed structure is much robust and could extend to other competitions that are not within the training dataset. 

% Besides that, we also demonstrate the ranking results on the other categories of figure skating. In Figure~\ref{fig:MS ranking} and Figure~\ref{fig:PF ranking}, results of mens short program and pairs free skating are shown, respectively. We also compared the model trained on Fis-V~\cite{xu2019learning} and FS1000 datasets. The model trained on the FS1000 dataset could achieve better results since FS1000 contains multiple categories while Fis-V only has one. Training on the FS1000 dataset allows the model to be more general and have better performance across different categories of figure skating. The model trained on the Fis-V dataset only has a sound result on ladies short program since Fis-V only contains that category. However, in the real scene, a general model that fits for various types of figure skating is more practical and useful. It also provides a possible idea that pre-training on the multi-category datasets and fine-tuning on a specific category might yield even better performance. This is worth further discussion in future work.
%However, for top athletes who get much higher score than others, the score difference would not affect the rankings much; for those athletes who have similar scores, the model may have different results. %More accurate methods are still needed.



==> LaTeX/Section/05_Experiment/visualization.tex <==
\subsection{Visualization}
\begin{figure}[h]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=1.0\linewidth]{LaTeX/image/visualization1.pdf}
\end{center}
\vspace*{-10pt}
    \caption{Score difference when sequentially adding clips. The score is low when the action is failed (blue box); the score is relatively high when finishing a complex move (yellow box) or skate fluently with the music (green box).}
\label{fig:visualization}
\vspace{-10pt}
\end{figure}
\noindent{In this section, we will demonstrate how our model scores in a certain video. We produce scores starting with the first clip and add one following clip at each time. When adding one clip, the score difference is computed to show the score of this clip. An example is shown in Figure~\ref{fig:visualization}. It can be seen that when an action is failed, the score for this clip is much lower (blue box). When the athlete successfully performs a complex technical move, the score is much higher (yellow box). Also, we found that when the athletes skate with the beat of the music, they also get higher scores (green box). This result clearly demonstrates that our proposed method could learn some basic patterns in figure skating.}

==> LaTeX/Section/06_Conclusion/manuscript.tex <==
%This paper introduces a comprehensive large-scale figure skating dataset and an MLP-based Skating-Mixer framework to learn multimodal representation for learning to score figure skating videos.
This paper introduces the MLP-based multimodal architecture for scoring figure skating. 
The proposed model solves learning multimodal information in long videos, which is essential in this task.
Besides, an elaborated-designed dataset has been collected.
We set the benchmarks that compare our model with CNN-Based, LSTM-based and Transformer-Based methods on the Fis-V and our proposed FS1000 datasets.
The experiments show the effectiveness of our method, indicating MLP-based architecture is capable of the multimodal task. 
Furthermore, we apply our model on the 2022 Winter Olympics to verify the model's effectiveness and applicability.
\jf{However, this work mainly focuses on the figure skating. It would be an interesting point to extend the dataset and the method to other sports. Also, the pose information can be great supplementary to do action-based tasks, which can be used to improve the method in the future.}
%However, there are two issues we cannot still solve well right now. we argue that: 1) the pose information can be great supplementary to do action-based tasks, which is not utilized in this paper. 2) The audio-visual integration has not been completely integrated with such a simple method. Therefore, it still exists much room for improvements in our future work.

==> Section/04_Method/attentive_mlpmixer.tex <==
\subsubsection{Attentive MLP-Mixer.}
\begin{figure}[h]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \vspace*{-25pt}
\includegraphics[width=1.0\linewidth]{LaTeX/image/att_mlp.pdf}
\end{center}
% \vspace*{-15pt}
    \caption{%Example video frames and the percentage of each category
    Structure comparison between the original MLP-Mixer and the Attentive MLP-Mixer.}
\label{fig:att_mlp}
% \vspace{-20pt}
\end{figure}
After processing all the clips in the video, we could directly use the final memory token output for scoring. However, we still want the model could utilize more local information in each clip and have an exhaustive understanding on such long sequence.
In figure skating, every clip does not contribute equally to the final score. Some technical moves or falls can significantly affect the final result.
One solution is to collect all the $\texttt{[CLS]}$ tokens and input those tokens with position embeddings to another MLP-Mixer block. Directly using MLP-Mixer could implicitly find the important part of the performance. 
Additionally, we propose a new structure, Attentive MLP-Mixer, which explicitly allows our model focus more on the important clips. Unlike the original MLP-Mixer block which first mixes token feature and then mixes channel feature, our structure first input the tokens into channel-mixing MLP and utilize sigmoid activation function to obtain token weights. The weights are multiplied with the original feature input. After that, the resulted tokens are input into the token-mixing MLP for further results.
To be more specific, suppose $\mathbf{C}$ is the concatenated tokens:
\begin{equation}
    \mathbf{C} = [\texttt{CLS}_1 \texttt{CLS}_2 ... \texttt{CLS}_t]
\end{equation}
The attention MLP-Mixer could be described as follow:
\begin{equation}
    \begin{aligned}
    \mathbf{X} &= \mathbf{C} + PE_c\\
    \mathbf{Z}_{j, *}&=\mathbf{X}_{j, *}+\mathbf{W}_{2} \Phi \left(\mathbf{W}_{1} \text{Norm}(\mathbf{X}_{j, *})\right),\\
    \mathbf{U} &= \sigma(\mathbf{Z}) \odot \mathbf{C} \\
\mathbf{Y}_{*, i}&=\mathbf{U}_{*, i}+\mathbf{W}_{4} \Phi \left(\mathbf{W}_{3} \text{Norm}(\mathbf{U}_{*, i})\right),
    \end{aligned}
\end{equation}
where $\odot$ denotes the element-wise production. The structure is shown in Figure~\ref{fig:att_mlp}. We took the mean value of the resulted features and concatenate with the last memory token output. The final score is generated by a linear layer. 

==> Section/04_Method/mlpmixer.tex <==
% \vspace{-10pt}
\subsection{Preliminary: MLP-Mixer}
% \subsubsection{MLP-Mixer}

In~\cite{tolstikhin2021mlp}, an MLP-based architecture has been proposed in the computer vision area and shows that %exclusively multi-layer perceptrons are powerful enough to achieve excellent results on image classification tasks.
model organizing multi-layer perceptrons are powerful enough to achieve excellent results on image classification tasks.
Similar to Visual Transformer~\cite{dosovitskiy2020image}, input images for MLP-Mixer~\cite{tolstikhin2021mlp} are split into several non-overlapping patches and each patch is treated as a sequence token. 
MLP-Mixer contains several identical layers, and each layer contains two MLP blocks: channel-mixing MLP and token-mixing MLP. 
Channel-mixing MLP operates on the channel dimension of the input feature, allowing different channels to communicate with each other; token-mixing MLP operates on the token dimension, so information could flow across different tokens and communicate with each other. 
Each block contains two MLP layers, and one GELU~\cite{hendrycks2020gaussian} activation function (described as $\Phi$). Besides, skip connection is also applied in each block. 

To be more specific, suppose $\mathbf{X} \in \mathbb{R}^{S \times C}$ is a two-dimension input feature, where $S$ is the sequence length (number of tokens) and $C$ is the number of channels for each token. In each layer, the function could be represented as:
\begin{equation}
\begin{aligned}
\mathbf{U}_{*, i}&=\mathbf{X}_{*, i}+\mathbf{W}_{2} \Phi \left(\mathbf{W}_{1} \text{Norm}(\mathbf{X}_{*, i})\right),\\
% , & \text { for } i=1 \ldots C \\
\mathbf{Y}_{j, *}&=\mathbf{U}_{j, *}+\mathbf{W}_{4} \Phi \left(\mathbf{W}_{3} \text{Norm}(\mathbf{U}_{j, *})\right),
% , & \text { for } j=1 \ldots S
\end{aligned}
\label{MLP-Mixer}
\end{equation}
where $i$ ranges from $1 \ldots C$, and $j$ ranges from $1 \ldots S$. 
$\text{Norm}$ denotes LayerNorm~\cite{ba2016layer} and $\mathbf{W}$ represents the weights of linear layer in each block. Input feature first passes through token-mixing MLP and then follows channel-mixing MLP.
% According to the author, it is unnecessary to use position encoding since token-mixing MLP is able to detect the order of input tokens.
This structure allows each element in the input feature could interact with other features along two dimensions.
